A Bayesian workflow for securitizing casualty insurance risk

Casualty insurance-linked securities (ILS) are appealing to investors because the underlying insurance claims, which are directly related to resulting security performance, are uncorrelated with most other asset classes. Conversely, casualty ILS are appealing to insurers as an efficient capital management tool. However, securitizing casualty insurance risk is non-trivial, as it requires forecasting loss ratios for pools of insurance policies that have not yet been written, in addition to estimating how the underlying losses will develop over time within future accident years. In this paper, we lay out a Bayesian workflow that tackles these complexities by using: (1) theoretically informed time-series and state-space models to capture how loss ratios develop and change over time; (2) historic industry data to inform prior distributions of models fit to individual programs; (3) stacking to combine loss ratio predictions from candidate models, and (4) both prior predictive simulations and simulation-based calibration to aid model specification. Using historic Schedule P filings, we then show how our proposed Bayesian workflow can be used to assess and compare models across a variety of key model performance metrics evaluated on future accident year losses.

==> src/prior-sensitivity.tex <==
\section{Prior sensitivity analysis}

We conducted a prior sensitivity analysis by running the full backtest pipeline as described in 
Section \ref{section:ledger-workflow} with either: (1) more diffuse priors, or (2) more informative
priors. The diffuse priors models scaled the prior standard deviations from the afforementioned 
section by 2.0, whereas the informative priors models scaled the prior standard deviations by 0.5. 
We chose these scaling factors because they represent significant changes in prior uncertainty, but 
still assume reasonable values that do not create degenerate model predictions.

Figure \ref{fig:scores-diffuse} shows model performance results for the diffuse prior model, and 
Figure \ref{fig:scores-inform} for the more informative variant. Overall, the results are very 
consistent across prior specifications. This is largely to be expected, in part because the 
hierarchical structure of the forecasting models makes the workflow quite robust to the specific
choice of prior on group-level parameters. With enough programs in each group (approximately 50 per 
line of business in this case), the group-level distribution is largely dominated by the data.

For completeness, we also show the posterior predictive checks for each of the diffuse and informed
prior models in Figures \ref{fig:posterior-diffuse} and \ref{fig:posterior-inform}, respectively. Recall 
that these results are on the ultimate losses for each accident year as predicted from the stacked 
forecasting model predictions. Comparing to Figure \ref{fig:posterior} in the main text, we see that the 
posterior predictions are themselves quite similar across the prior specifications.

\renewcommand{\thefigure}{A\arabic{figure}}
\setcounter{figure}{0}

\begin{figure}[t!]
    \centering
    \includegraphics[scale=.5]{\figures/scores-diffuse}
    \caption{
        ELPD (left) and RMSE (right) differences (+/- 2 standard errors) for the diffuse
        prior models, ordered by Validation dataset performance for each model and line of business.
    }
	\label{fig:scores-diffuse}
\end{figure}

\begin{figure}[t!]
    \centering
    \includegraphics[scale=.5]{\figures/scores-inform}
    \caption{
        ELPD (left) and RMSE (right) differences (+/- 2 standard errors) for the more informative
        prior models, ordered by Validation dataset performance for each model and line of business.
    }
	\label{fig:scores-inform}
\end{figure}

\begin{figure}[t!]
    \centering
    \includegraphics[scale=.5]{\figures/posterior-predictions-CA-diffuse}
    \caption{
        Posterior predictions for three random commercial auto programs from the 
        \cite{meyers2015} dataset, under the diffuse prior specification. The programs 
        here are the same as in Figure \ref{fig:posterior}. The shaded regions correspond to the 50\% and 95\% credible intervals for the predictions, and points are true losses at $y_{i(10)}$.
    }
	\label{fig:posterior-diffuse}
\end{figure}


\begin{figure}[t!]
    \centering
    \includegraphics[scale=.5]{\figures/posterior-predictions-CA-inform}
    \caption{
        Posterior predictions for three random commercial auto programs from the 
        \cite{meyers2015} dataset, under the informed prior specification. The programs 
        here are the same as in Figure \ref{fig:posterior}. The shaded regions correspond 
        to the 50\% and 95\% credible intervals for the predictions, and points are true losses at $y_{i(10)}$.
    }
	\label{fig:posterior-inform}
\end{figure}
